Local Label Propagation for Large-Scale Semi-Supervised Learning

A significant issue in training deep neural networks to solve supervised learning tasks is the need for large numbers of labelled datapoints. The goal of semi-supervised learning is to leverage ubiquitous unlabelled data, together with small quantities of labelled data, to achieve high task performance. Though substantial recent progress has been made in developing semi-supervised algorithms that are effective for comparatively small datasets, many of these techniques do not scale readily to the large (unlaballed) datasets characteristic of real-world applications. In this paper we introduce a novel approach to scalable semi-supervised learning, called Local Label Propagation (LLP). Extending ideas from recent work on unsupervised embedding learning, LLP first embeds datapoints, labelled and otherwise, in a common latent space using a deep neural network. It then propagates pseudolabels from known to unknown datapoints in a manner that depends on the local geometry of the embedding, taking into account both inter-point distance and local data density as a weighting on propagation likelihood. The parameters of the deep embedding are then trained to simultaneously maximize pseudolabel categorization performance as well as a metric of the clustering of datapoints within each psuedo-label group, iteratively alternating stages of network training and label propagation. We illustrate the utility of the LLP method on the ImageNet dataset, achieving results that outperform previous state-of-the-art scalable semi-supervised learning algorithms by large margins, consistently across a wide variety of training regimes. We also show that the feature representation learned with LLP transfers well to scene recognition in the Places 205 dataset.

==> sections/methods_back.tex <==
Our overall purpose is to map pixel representations of images to lower-dimensional representations where images with the same label are closer and images with different labels are relatively further. To be concrete, the objective of our work is to learn a parametric map $f_\theta(\cdot)$ that embeds pixel representations of images in a D-dimension embedding space: $v_i=f_\theta(x_i)$. Each iteration of our method consists of the following two steps:
\begin{itemize}
    \item Optimize the parametric representation based on learned pseudo-labels and the confidence of each pseudo-label in order to make the embeddings of images with the same label closer. 
    \item Update pseodo-labels and the corresponding confidences based on the learned representation, in other words, propagate labels to unlabeled images according to their $K$ nearest labeled neighbours in the embedding space.
\end{itemize}

We have two strategies to utilize our model to do the image classification task. The first strategy is transfer learning. We fix the finally learned representation network and train a fully-connected network upon a certain layer of it. The second strategy is to include the classification loss as training the representation network. 

\color{red}
(Method overview: iterative representation learning and label propagation using learning representations. Mention that label propagation gets both pseudo-labels and confidence. Classifier learning at the same time or afterwards.)\color{black}

\subsection{Representation Learning}
We formulate the loss function which measures the aggregation of images with the same label based on a non-parametric softmax operation proposed by Wu et al. In that work, the aothors define the probability that an arbitrary feature $v$ is recognized as the $i$-th image to be:
\begin{equation}
P(i|v)=\frac{exp(v_i^Tv/\tau)}{\sum_{j=1}^Nexp(v_j^Tv/\tau)},
\label{softmax}
\end{equation}
where temperatue $\tau\in [0,1]$ is a fixed hyperparameter, $N$ is the total number of images, $v$ and $\{v_i\}$ are all L2 normalized vector ($||v||_2=1$) in the D-dimension embedding space. Following Eq. \ref{softmax},  given an image set $S$, we then define the probability of embedding $v$ being recognized as an image in $S$ as:
\begin{equation}
    P(S|v)=\sum_{i\in S}P(i|v).
    \label{sum_softmax}
\end{equation}

Based on the formulations above, we define the aggregation loss as:
\begin{equation}
  loss_a = -\log P(A|v),  
  \label{loss_a}
\end{equation}
where $v$ is the current representation, $A$ is the set of images that share the same pseudo-labels with $v$.

For the purpose of enhancing the final classification performance, we found that adding a classifier head upon the representation network can be helpful. The classification loss is characterized by the cross-entropy loss:
\begin{equation}
    loss_c = -\log \frac{exp(s_{y})}{\sum_{j=1}^M exp(s_j)},
    \label{loss_c}
\end{equation}
where $y$ is the ground truth label, $\{s_i\}$ are scores predicted by the classifier, $M$ is the number of labels. Note that only labeled images are used to train the classifier.

Finally, the total loss function to be minimized in representation learning is defined as:
\begin{equation}
    loss = c \cdot (loss_a + loss_c) + \lambda ||\theta||^2,
    \label{loss_total}
\end{equation}
where $c$ is the confidence of the pseudo-label of the current image which will be explained in the next subsection weighting on the loss function, $\lambda$ is the L2 regularization hyperparameter.

\color{red}
(The basic non-parametric softmax setting, should include the local aggregation paper equation 1 and equation 2.)

(Pseudo-labels and optimization goal: maximizing P(A|v), where A is the set of images sharing the same pseudo-label. Describe the negative log-likelihood of P(A|v) as the loss to be minimized.)

In practice, we find that training a classifier on the pseudo-labels helps the final performance. (Describe the other head and the cross-entropy loss)

(Give the final loss function, mention that they are weighted by the confidence. c * (-log P(A|v) + category loss) + weight decay)
\color{black}

\subsection{Label Propagation}
We identify a pseudo-label for each image in the batch in every iteration. If an image is a labeled image, its pseudo-label will be simply its true label. If an image is unlabeled, its pseudo-label will be identified by weighted voting among its top $K$ nearest labeled neighbors, where cosine similarity is used to measure any two images' distance (larger $v_i^Tv_j$ is, closer the two images are). Each image among the top $K$ nearest labeled neighbors votes for its own label weighted by the (normalized) exponential cosine similarity between itself and the current representation :
\begin{equation}
    p_i=\frac{exp(w_i^Tv)}{\sum_{j=1}^K exp(w_j^Tv)},
    \label{weight}
\end{equation}
where $\{w_1...w_K\}$ are the top $K$ nearest labeled neighbors of $v$. Therefore, the total votes for each label are given by:
\begin{equation}
    P_m = \sum_{i=1}^K \mathbbm{1}(label(i)=m)\cdot p_i,
    \label{vote}
\end{equation}
where $\mathbbm{1}$ is the indicator function, $m=1,2...M$, $label(i)$ is the label of $w_i$. Then the identified label and its confidence are given by
\begin{equation}
    \tilde{m}=\argmax_m P_m,
    \label{pseudo_label}
\end{equation}

\begin{equation}
    c=P_{\tilde{m}},
    \label{confidence}
\end{equation}
respectively.

The formulations above only consider cosine similarities between the current image and its labeled neighbors, ignoring the neighborhood of these labeled images. Intuitively, denser the neighborhood of a labeled image is, lesser the possibility that the current image shares the same label with it. Assuming that this intuition is correct, we introduce an extra local weight for each labeled image. We modify Eq. \ref{weight} as:
\begin{equation}
    p_i=\frac{exp(w_i^Tv)}{\sum_{j=1}^K exp(w_j^Tv)}\cdot \frac{1}{\sum_{l=1}^{K^{LW}}exp(w_i^Tu_l)},
    \label{LW_weight}
\end{equation}
where $K^{LW}$ denotes the number of nearest neighbors of $w_i$ we consider, $\{u_l\}$ are embedding vectors of the top $K^{LW}$ nearest neighbors of $w_i$. In this setting, the top $K$ nearest labeled neighbors of the current image are chosen based on Eq. \ref{LW_weight} instead of the cosine similarity, and Eq. \ref{vote}, Eq. \ref{pseudo_label}, Eq. \ref{confidence} still hold true. In practice, we found that the local weight approach does indeed improve the performance.

\color{red}(Basic formulation about top K nearest neighbor in labeled images for identifying neighbors. Give formulations about both the pseudo-labels and confidence.)

(Local weight. First describe why it's needed, then describe its formulation. Finally give new formulations of pseudo-labels and confidence based on local weight.)\color{black}

%\subsection{Classifier Learning}
%If the classification loss is not included in the representation learning, we do transfer learning after the representation learning. To be concrete, we fix the representation network and add an average pooling layer and a fully-connected layer sequentially upon a certain layer of the representation network as the classifier. We train the classifier on images with true labels.

%\color{red}(How we train the classifier afterwards.)\color{black}

==> sections/tables/res18_res50.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{c|c|c}
\hline
Method & ResNet-18 & ResNet-50 \\
\hline\hline
100\% Supervised & 70.53 &  75.98 \\
10\% Supervised & 47.89 & 56.35 \\
\hline
DCVT~\cite{} & 53.50 & -- \\
MT* & 55.65 & 64.31 \\
\ShortName (ours) & \textbf{61.51} & \textbf{68.91} \\
\hline
\end{tabular}
\end{center}
\caption{
Top-1 accuracy (\%) on ImageNet validation set for different architectures trained on ImageNet using 10\% labels.
*: Mean teacher performance is produced by us.
}
\label{tab:res18_50}
\vspace{-2mm}
\end{table}
